Clustering and Cliques in P.A random graphs with edge insertion

In this paper, we investigate the global clustering coefficient (a.k.a transitivity) and clique number of graphs generated by a preferential attachment random graph model with an additional feature of allowing edge connections between existing vertices. Specifically, at each time step $t$, either a new vertex is added with probability $f(t)$, or an edge is added between two existing vertices with probability $1-f(t)$. We establish concentration inequalities for the global clustering and clique number of the resulting graphs under the assumption that $f(t)$ is a regularly varying function at infinity with index of regular variation $-\gamma$, where $\gamma \in [0,1)$. We also demonstrate an inverse relation between these two statistics: the clique number is essentially the reciprocal of the global clustering coefficient.

==> bounds_degree.tex <==
% !TeX root = ms.tex
\section{Proof Technical Estimates}

This section is devoted to provide bounds for vertices' degree as well as the asymptotic behavior of some particular functions that will play important roles in our proofs. We begin by obtaining estimates for the degrees and finish this section with analytical results about some functions of $f$. 

\subsection{Lower bound for maximum degree}In this section we will prove a useful lower bound for the maximum degree of $G_t(f)$. Our general strategy will be to apply the results obtained for the function identically equal to~$p$, with $p \in (0,1)$ (which we denote by~$\mathrm{cons}_p$) in \cite{ARS17} and propagate them to smaller functions via the doubly-labeled random tree process. 

For the sake of the reader's convenience, we state and comment the aforementioned results here. Given~$m\in\Z_+$, we order the vertices of~$G_t(\mathrm{cons}_p)$ from oldest to earliest and then divide them into blocks of size~$m$. We then denote by~$d_{t,m}(j)$ the sum of all degrees of the vertices from the~$j$-th block. The following theorem has a involved notation, but in essence it provides with high probability an explicit polynomial lower bound for~$d_{t,m}(j)$. 
\begin{theorem}[Theorem 2 from~\cite{ARS17} ] \label{teo:cotainf} Given~$p\in(0,1]$, let~$\xi\in(0,2(2-p)^{-1}-1)$ and fix $m\in\Z_+$ sufficiently large. Define
	\begin{equation*}
	\zeta_m:=\frac{(1-p)}{2(2-p)m^{\xi}}.
	\end{equation*} 
	and let 
	\[
	1 < R < m(1-p/2)(1-\zeta_m).
	\] 
	There exists a positive constant $c = c(m, R, p)$ such that, for \[\beta\in(0,(1-p/2)(1-\zeta_m)) \textit{ and } j \geq m^{\frac{2}{1-p}} + 1,\] we have
	\begin{equation}
	\label{eq:teocliqp}
	\P\left( d_{t,m}(j) < t^{\b} \right) \le c\frac{j^R}{t^{R-\b R(1-p/2)^{-1}(1-\zeta_m)^{-1}}} +\frac{m}{[(j-1)m]^{99}} .
	\end{equation}
\end{theorem}


\begin{proposition}\label{prop:grauinf} Let $f$ be an edge-step function decreasing to zero. Then, for any $\varepsilon \in (0,1)$ there exist positive constants $c_1,c_2$ and $c_3$ depending on $\varepsilon$ and $f$ only such that
    $$
    \Pd \left(\exists v \in G_t(f) \; : \; d_t(v) \ge c_1t^{1-\varepsilon}\right) \ge 1 - c_2t^{-c_3}.
    $$
\end{proposition}
\begin{proof} The proof will follow from Theorem \ref{teo:cotainf} together with Proposition \ref{p:diammaxdegProp}. 

 Notice that we can assume w.l.o.g that for a given $p$, $f(t) \le p$ for all $t$. \notarodrigo{Explicar!!!}

 Given $\varepsilon$, choose $p$ small enough and $m$ large enough in order to
 $$
\beta := \left(1-\frac{\varepsilon}{2}\right)\left(1-\frac{p}{2}\right)\left(1-\zeta_m\right) \ge 1-\varepsilon.
 $$
Setting $j=t^{\varepsilon/4}$, the above choices in \eqref{eq:teocliqp} lead to
$$
\P\left( d_{G_t(\mathrm{cons}_p),m}(j) < t^{1-\varepsilon} \right) \le c\frac{1}{t^{R\varepsilon/4}} +\frac{m}{t^{99\varepsilon/4}}. 
$$
Thus, w.h.p, by the pigeonhole principle the maximum degree of $G_t(\mathrm{cons}_p)$, for $p$ small enough is at least $t^{1-\varepsilon}/m$. Finally, by Proposition \ref{p:diammaxdegProp} it follows that the maximum degree of $G_t(f)$ is at least $t^{1-\varepsilon}/m$ as well. This concludes the proof.
\end{proof}

\subsection{Upper bound for vertices' degrees} It will be useful to our purposes to have an upper bound the degree of a given vertex. In order to state properly the next result, given an edge-step function $f$ and $i\in \N$, we will denote by $\tau_i$ the time the process $\{G_t(f)\}_{t\ge 0}$ adds its $i$-th vertex. We will also define the following functions
\begin{equation}\label{def:phi}
    \phi(t) := \prod_{s=1}^{t-1}\left(1 + \frac{1}{s} - \frac{f(s+1)}{2s}\right).
\end{equation}
and for $f$ strictly positive we let $F^{-1}:\R\to\R$ be the following function
\begin{equation}
\label{eq:Finvdef}
 F^{-1}(r):=\inf_{s \in \R}\{     F(s) \geq r \}.
\end{equation}
Notice for this regime of $f$ and since~$\|f\|_\infty \leq 1$, we have that
\begin{equation}\label{eq:Finvdef2}
r\leq F(F^{-1}(r))\leq r+1,\quad\text{ and } \quad r\leq F^{-1}(F(r))\leq r+1.
\end{equation}
Finally, we also let $\phitil$ be the following function
\begin{equation}\label{def:phitil}
	\phitil(s):= \phi(F^{-1}(s))
\end{equation} 
With the above notation in mind we state the following results
\begin{lemma}[Lemma 3.6 in (?)]\label{l:upperbounddeg}Let $f$ be an edge-step function that decreases to zero. Then, there exist positive constants $c_1$ and $c_2$ depending on $f$ only such that, for any $i, n \in \N$ and any $\alpha >1$
    $$
        \Pd \left( \exists t\ge n, \; d_t(i) \ge \alpha \frac{\phi(t)}{\phi(n)} \; \middle |\; \tau_i = n\right) \le c_1 \exp \{ - c_2\alpha\}.
    $$
    
\end{lemma}
In the light of the above lemma, we now work in the direction of obtaining an analogous bound without the dependence on~$\tau_i$. The idea is elementary: the variable $\tau_i$ concentrates strongly around its mean, so paying a small price we may ignore all possible times~$n$ that are far away from said mean. Our next result uses this fact in order to obtain a concentration result for~$\tau_i$ with high probability.
\begin{lemma}
\label{lemma:tauibound}
Consider~$f$ either in~$\mathrm{RES}(\gamma)$ with~$\gamma\in[0,1)$ or identically equal to~$p\in(0,1]$. Then there exists a constant~$C_f>0$ such that for~$i\in\N$ and every~$\delta>0$,
\begin{equation}
\label{eq:tauiconc}
\P\left((1-\delta)F^{-1}(i)\le \tau(i)     \leq  (1+\delta)F^{-1}(i)     \right) \ge 1- C_f^{-1}\exp\left\{   -C_f  (1-\gamma)\delta  i      \right\}.
\end{equation}
\end{lemma}
\begin{proof}
If~$f\equiv p$, then the result follows by an elementary Bernstein bound. Assume then that~$f\in \mathrm{RES}(\gamma)$. We will prove that there exist a constant $C'_f$ such that 
\begin{equation}\label{eq:taulower}
	\P\left( \tau(i)     \leq  (1-\delta)F^{-1}(i)     \right) \le (C'_f)^{-1}\exp\left\{   -C'_f  (1-\gamma)\delta  i      \right\}.
\end{equation}
The upper bound for the probability of the event $\{\tau(i) \ge (1+\delta)F^{-1}(i)\}$ will follow from the exactly same argument.

By Theorem \ref{thm:repthm}, we know that~$f(t)=\ell(t)t^{-\gamma}$ with~$\ell$ being a slowly varying function. Proposition \ref{prop:factorout} implies that as~$r\to\infty$, using the monotonicity of~$f$ to approximate the integral by the sum,
\begin{equation}
\label{eq:cotaF2}
\begin{split}
F((1-\delta)r)
 &=\sum_{s=1}^{\lfloor  (1-\delta) r  \rfloor}      f(s)   \\  
  & =  \sum_{s=1}^{\lfloor (1-\delta) r   \rfloor}      \ell(s)s^{-\gamma}   \sim \frac{1}{1-\gamma}\ell((1-\delta) r)(1-\delta)^{1-\gamma}r^{1-\gamma} \\
  & \sim (1-\delta)^{1-\gamma} F(r),
\end{split}
\end{equation}
where we also used the fact that~$\ell$ is slowly varying to obtain~$\ell((1-\delta)r)\sim\ell(r)$. Letting $i_* = (1-\delta)F^{-1}(i)$
and recalling that~$V_r(f)$ is a sum of independent random variables, we may use the above equation, \eqref{eq:Finvdef2}, and an elementary Chernoff bound to obtain
\begin{equation}
\label{eq:tauiconc2}
\begin{split}
\lefteqn{\Pd\left(\tau(i)     \leq  (1-\delta)F^{-1}(i)     \right)}\quad\quad
\\
&=
\Pd\left( V_{i_*}(f)  \geq i     \right)
\\
&=
\Pd\left( V_{i_*}(f)  \geq \left(1+\left(i \left( F\left((1-\delta)F^{-1}(i)\right)\right)^{-1}-1\right)\right)\Ed\left[  V_{i_*}(f)       \right]    \right)
\\
&\leq 
\exp\left\{   -\frac{1}{3}   \left(i \left( F\left((1-\delta)F^{-1}(i)\right)\right)^{-1}-1\right)  F\left( (1-\delta)F^{-1}(i)\right)          \right\}
\\
&\leq 
\exp\left\{   -\frac{1}{3}  \left(   (1-\delta)^{-(1-\gamma)}      -1\right)(1-\delta)^{1-\gamma} \cdot i      \right\}
\\
&\leq 
\exp\left\{   -C(1-\gamma)\delta i      \right\},
\end{split}
\end{equation}
for sufficiently large~$i$. By adjusting the constant we can then show~\eqref{eq:taulower} for every~$i\geq 1$. 

To prove an upper bound of same order for $\Pd \left( \tau(i) \ge (1+\delta)F^{-1}(i)\right)$. Just notice the estimate given at \eqref{eq:cotaF2} also holds replacing $(1-\delta)$ by $(1+\delta)$. That is, $F(1+\delta)r) \sim (1+\delta)^{1-\gamma}F(r)$. Then, the exactly same reasoning we have done applies since the identity of events below holds
$$
\{\tau(i) \ge (1+\delta)F^{-1}(i)\} = \{V_{(1+\delta)F^{-1}(i)}(f) \le i\}.
$$
This concludes the proof.
\end{proof}
We can now prove the next result:
\begin{theorem}\label{thm:upperbounddeg2}
	Consider~$f$ either in~$\mathrm{RES}(-\gamma)$ with~$\gamma\in[0,1)$ or identically equal to~$p\in(0,1]$. Then there exists a constant~$C_f>0$ such that, for every~$\alpha>1$,
	\begin{equation*}
	\label{eq:upperbounddeg2}
	\begin{split}
	\P\left(       \exists s\in\N \text{ such that } d_s(i) \geq   \alpha\frac{\phi(s)}{\phitil(i)}                     \right) & \leq C_f^{-1}\left(\exp\left\{   -C_f \frac{\alpha-1}{\alpha} i    \right\}     +  \exp\left\{   -C_f \cdot  \alpha    \right\} \right)    . 
	\end{split}
	\end{equation*}
\end{theorem}
\begin{proof}
We first assume that $f\in\mathrm{RES}(\gamma)$. We note that, for~$r>0$ and~$\delta\in(0,1)$,
\begin{equation}
\label{eq:phiFphiFsobre2}
\frac{\phi\left(r\right)}{\phi\left((1-\delta)r\right)}=\prod_{s=(1-\delta)r}^{r-1}
\left(     1+\frac{1}{s}              -\frac{f(s+1)}{2s}       \right) \leq 
\prod_{s=(1-\delta)r}^{r-1}
  \frac{s+1}{s}       \leq \frac{1}{1-\delta}.       
\end{equation}
Let~$\delta = (\alpha-1)/(2\alpha)$, so that~$\alpha(1-\delta)>1$ and~$\delta\in(0,1)$. We obtain, by the above equation, monotonicity, and the union bound,
\begin{equation}
\label{eq:upperbounddeg3}
\begin{split}
\lefteqn{\P\left(       \exists s\in\N \text{ such that } d_s(i) \geq   \alpha\frac{\phi(s)}{\phitil(i)}              \right) }\phantom{**}
\\
&\leq  
\P\left(\tau(i)     \leq \left(1 -\delta\right) F^{-1}(i)     \right)
\\
&\quad +
\P\left(       \exists s\in\N \text{ such that } d_s(i) \geq   \alpha(1-\delta)\frac{\phi(s)}{\phi\left((1-\delta)F^{-1}(i)\right)}  \middle |  \tau(i)     = (1-\delta)F^{-1}(i)           \right),
\end{split}
\end{equation}
The result for~$f\in\mathrm{RES}(\gamma)$ then follows after using lemmas~\ref{l:upperbounddeg} and~\ref{lemma:tauibound}. For~$f\equiv p$, Theorem~$3$ of~\cite{ARS19c} already implies the result.
\end{proof}

We note that the bound in~\eqref{eq:upperbounddeg2} is sharp in the sense that the order of~$\Ed[d_s(i)]$ is already~$\phi(s)/\phi(F^{-1}(i))$. 

\subsection{Asymptotic behavior of $\phi, F, F^{-1}$ and other related functions} This subsection is a technical one and can be skipped in a first reading. Throughout this subsection we will assume $f$ satisfies condition \eqref{def:conditionRV} with $\gamma \in [0,1)$. For this reason, most of the results here rely on results coming from the Karamata's theory of the regularly varying functions. The reader may find the more classical results stated in the Appendix.

Recall the definition of $\phi$ given at \eqref{def:phi}. Then, we have the following characterization result
\begin{lemma}\label{lemma:phixi}Let $f$ be an edge-step function decreasing to zero. Then, there exists a slowly varying function at infinity $\xi$ such that
	$$
	\phi(s) = \xi(s)s.
	$$
\end{lemma}
When $f$ is regularly varying we can use the Karamata Theory to obtain results for the asymptotic behavior of $F$ and its generalized inverse $F^{-1}$.
\begin{lemma}\label{lemma:F}Let $f$ be an edge-step function satisfying condition \eqref{def:conditionRV} with $\gamma \in [0,1)$. Then, $F$ is a regularly varying function of index $1-\gamma$. Moreover, there exist a slowly varying function $\ell_1$ such that
	$$
		F(t) = \ell_1(t)t^{1-\gamma}.
	$$
\end{lemma}
\begin{proof} By Theorem~\ref{thm:repthm}, there exists a slowly varying function $\ell'$ such that $f(s) = \ell'(s)s^{-\gamma}$. Using that $f$ is decreasing, we have
	$$
	1+\int_{1}^tf(s)\mathrm{d}s  \le F(t) \le 1+ \int_{0}^tf(s)\mathrm{d}s 
	1+
	$$
	On the other hand, by Proposition \ref{prop:factorout}
	$$
	\int_{t_0}^tf(s)\mathrm{d}s \sim \frac{1}{1-\gamma}\ell'(t)t^{1-\gamma},
	$$
	which implies $F(t) \sim \frac{1}{1-\gamma}\ell'(t)t^{1-\gamma}$ and that $F$ is regularly varying with index $1-\gamma$. Applying Theorem \ref{thm:repthm} we finally have that there exists $\ell_1$ such that $F(t) = \ell_1(t)t^{1-\gamma}$.
\end{proof}
From the above lemma and Theorem \ref{thm:inverse} we obtain the following result
\begin{lemma}\label{lemma:finverse}Let $f$ be an edge-step function satisfying condition \eqref{def:conditionRV} with $\gamma \in [0,1)$. Then, there exists a slowly varying function $\ell$ such that
	$$
	F^{-1}(s) = \ell_2(s)s^{\frac{1}{1-\gamma}}.
	$$
\end{lemma} 
Recall the definition $\phitil$ in \eqref{def:phitil}. Then, the lemma below is a consequence of the above lemmas
\begin{lemma}\label{lemma:phitil}Let $f$ be an edge-step function satisfying conditions \eqref{def:conditionD0} and \eqref{def:conditionRV} with $\gamma \in [0,1)$. Then, there exist a slowly varying function $\widetilde{\ell}$ such that
	$$
	\phitil(s) = \widetilde{\ell}(s)s^{\frac{1}{1-\gamma}}.
	$$
\end{lemma}



==> decoupling.tex <==
% !TeX root = ./ms.tex
\section{Decoupling number of edges between vertices}
Estimating the expected value of some particular type of subgraph such as triangles becomes much harder in the presence of the edge-step when compared with the same task in the BA-model (see \cite{BR04}). The reason is that a particular subgraph $H$ induced by a fixed set of vertices can be constructed in many ways and times, since we combine edges created by edge-steps with the ones created by vertex-steps. \notarodrigo{expand...or discuss it in the techinical ideas}

Throughout this section we will always assume $f$ to be in \eqref{def:conditionRV} for $\gamma \in [0,1)$. We will also use letters $i,j$ and $k$ to denote the $i$-th, $j$-th and $k$-th vertices added by $\{G_t(f)\}_{t\ge 0}$. Moreover, for a pair $i$ and $j$ and a specific time $s$, we let $e^{i,j}_s$ and $g_s^{i,j}$ be the following random variables
\begin{align}
	\label{eq:edgeind}
	\es{s}{i}{j} &:=\mathbb{1}\{\text{an edge is added between }i\text{ and }j\text{ at time } s \text{ by an edge-step }  \},
	\\ \nonumber
	\vs{s}{i}{j} &:=\mathbb{1}\left\{
	\text{an edge is added between }i\text{ and }j\text{ before time } t \text{ and by a vertex-step}
	\right\}.
\end{align}
We use the $f$-dependent constant $C_f$ in the statement of Theorem \ref{thm:upperbounddeg2}, to define for $s \in [t]$ and $i,j \in [t]$ the following functions
\begin{equation}
	\label{eq:pijdef}
	p^{i,j}_s :=  \frac{100(\log t)^2 \phi(s)^2}{[C_f(1-\gamma)]^2\phitil(i)\phitil(j)s^{2}} \wedge 1
	\end{equation}
and 
	\begin{equation}
	\label{eq:qijdef}
	q^{i,j} :=  
		\frac{5\log t}{C_f(1-\gamma)\phitil(i)}\wedge 1.	
	\end{equation} 
The terms $p_s^{i,j}$ and $q^{i,j}$ are related to the random variables $\es{s}{i}{j}$ and $\vs{i}{j}$ in the way given by the lemma below.
\begin{lemma}\label{lemma:negativecor} Let $f$ be an edge-step function in \eqref{def:conditionRV}, for $\gamma \in [0,1)$. Then, given $t \ge 0$, any triplet of vertices $  i,j,k \in \{ 10(C_f(1-\gamma))^{-1}\log t, \dots, t\}$ and times~$r,s,s'\in [t]$, there exists a positive constant $C_1$ depending on $f$ only such that the following holds
	\begin{enumerate}
		\item[(a)] 
		\begin{equation*}
			\Ed \left[ \vs{i}{j}\vs{i}{k}\right] \le C_1 q^{i,j}q^{i,k}; \quad \Ed \left[ \es{r+1}{i}{j}\vs{i}{k}\right] \le C_1 p^{i,j}_rq^{i,k}; \quad \Ed \left[ \es{r+1}{i}{j}\es{s+1}{i}{k}\right] \le C_1 p^{i,j}_rp^{i,k}_s;
			\end{equation*}
		\item[(b)]
	\begin{gather*}
		\Ed \left[ \vs{i}{j}\vs{i}{k}\es{s'+1}{j}{k}\right] \le C_1 q^{i,j}q^{i,k}p^{j,k}_{s'}; \quad \Ed \left[ \vs{i}{j}\es{s+1}{i}{k}\es{s'+1}{j}{k}\right] \le C_1 q^{i,j}p^{i,k}_sp^{j,k}_{s'} \\
		\Ed \left[ \es{r+1}{i}{j}\es{s+1}{i}{k}\es{s'+1}{j}{k}\right] \le C_1 p^{i,j}_rp^{i,k}_sp^{j,k}_{s'}.
	\end{gather*}
	\end{enumerate}
\end{lemma}
Before we prove the above lemma let us say some words about its statement. Notice that using the dynamics of the process $\{G_t(f)\}_{t\ge 0}$ we have that
\begin{equation}\label{eq:expees}
    \Ed\left[ \es{s+1}{i}{j} \, \middle |\, \mathcal{F}_s\right] = (1-f(s+1))\frac{d_s(i)d_s(j)}{2s^2}.
\end{equation}
Now, by Equation (2.3) in [ARS20diam] and Lemma \ref{lemma:tauibound} it follows that 
$$
\Ed \left[d_s(i)\right] = \Theta\left( \frac{\phi(s)}{\phi(F^{-1}(i))} \right).
$$
Observe that if the degree of the $i$-th vertex behaves like its expectation, returning to Equation \eqref{eq:expees}, we would have that, up to a power of $\log t$, $\Ed[\es{s+1}{i}{j}]$ looks like $p_s^{i,j}$. The same reasoning could be carried over to~$\Ed[\vs{i}{j}]$, replacing $p_s^{i,j}$ by $q^{i,j}$. 

Although, we do not have lower bound for $d_s(i)$ as sharp as the upper given by Lemma \ref{l:upperbounddeg}, it may be instructive to think of $p_s^{i,j}$ (resp. $q^{i,j}$) as the expectation of $\es{s+1}{i}{j}$ (resp. $\vs{i}{j}$). From this perspective, the above lemma may be read as follows: up to a power of $\log t$, the random variables $\es{r}{i}{j}$ and $\vs{i}{j}$ are all negatively correlated. This approximated negative correlation will help us to obtain upper bound for the expected number of specific subgraphs in $G_t(f)$.

Now we can go to the proof of the result.
\begin{proof}[Proof of Lemma \ref{lemma:negativecor}]As usual, we start by introducing some definitions and establishing some notations. Throughout this proof we will assume $i<j<k$. 
%Additionally, enlarging our probability space if needed, we assume there exist an i.i.d sequence of uniformly distributed random variables $\{\mathcal{U}_s\}_{s\ge0}$ over $[0,1]$ and $\{\mathcal{U}^{i,j}\}_{i,j \in \{1,\dots,t\}}$, with the additional property of being independent of the random graph process $\{G_t(f)\}_{t\ge 0}$ and of each other. 


Recall from the definition of the random graph process $\{G_t(f)\}_{t\ge 0}$ the Bernoulli random variables $Z_s \eqd \mathrm{Ber}(f(s))$. We then define the following filtration
\begin{equation}
	\mathcal{G}_s := \sigma\left( \mathcal{F}_{s-1}, Z_s\right).
\end{equation}
% Then we introduce the random variables $\est{s}{i}{j}$ and $\vst{i}{j}$ as follows
% \begin{equation}
% 	\est{s}{i}{j} := \es{s}{i}{j} + (1-\es{s}{i}{j})\frac{\mathbb{1}\{\mathcal{U}_s \leq p^{i,j}_{s-1} - \Ed[ \es{s}{i}{j} \vert \mathcal{F}_{s-1} ] \}}{1- \Ed[ \es{s}{i}{j} \vert \mathcal{F}_{s-1} ]   }
% \end{equation}
% and 
% \begin{equation}
% 	\vst{i}{j} := \vs{i}{j} + (1-\vs{i}{j})\frac{\mathbb{1}\{\mathcal{U}^{i,j} \leq q^{i,j} - \Ed[ \vs{i}{j} \vert \mathcal{G}_{\tau(j)} ] \}}{1- \Ed[ \vs{i}{j} \vert \mathcal{G}_{\tau(j)} ]   }
% \end{equation}
% \notarodrigo{say some words about the intuition behind the above random variables}
% Before we proceed with the proof, let us briefly discuss the motivation behind the new random variables $\est{s}{i}{j}$ and $\vst{i}{j}$. The first observation is that for all $i,j$ and time $s$ these random variables are independent of each other. Moreover, by using an extra and independent randomness source (the sequence $\{\mathcal{U}_s\}_{s\ge0}$ and $\{\mathcal{U}^{i,j}\}_{i,j \in \{1,\dots,t\}}$) we give to $\est{s}{i}{j}$ and $\vst{i}{j}$ an extra chance of being~$1$. The upshot is that we have two new sequences of random variables with much simpler dependence relation and, as we will see latter, whose expected values are close to the expected value of the original ones.

%Note that the above variables are well-defined, since $f$ is positive and decreasing and, by \ref{eq:expees} and \eqref{eq:expecvs}, both~$ \Ed[ \es{s}{i}{j} \vert \mathcal{F}_{s-1} ]$ and $\Ed[ \vs{s}{i}{j} \vert \mathcal{F}_{s-1} ]$ are strictly smaller than $1$. 

Given a vertex $i$ and a fixed time $t$, it will be useful to introduce the following stopping time 
\begin{equation}
	\eta_{i}:=\inf_{s \in \N}\left\{d_s(i) \geq 10[C_f(1-\gamma)]^{-1} \log (t) \frac{\phi(s)}{\phitil(i)}     \right\},
\end{equation}
and for a triplet of vertices $i<j<k$ we let $\widetilde{\eta} = \eta_{i}\wedge\eta_{j}\wedge\eta_{k}$. 
% Moreover, we denote by $\widetilde{\mathcal{F}_s}$ the following sigma-algebra 
% $$
% \widetilde{\mathcal{F}_s} := \sigma\left(\mathcal{F}_s, \mathcal{U}_0, \dots, \mathcal{U}_s \right).
% $$
By the definition of $\widetilde{\eta}$ the following bound holds 
\begin{equation}\label{eq:esbound}
	\Ed\left[ \es{s+1}{i}{j} \mathbb{1}\{\widetilde{\eta} > s\}\middle | \mathcal{F}_s\right] = \mathbb{1}\{\widetilde{\eta} > s\}(1-f(s+1))\frac{d_s(i)d_s(j)}{2s^2} \le  p_s^{i,j}\mathbb{1}\{\widetilde{\eta} > s\}.
\end{equation}
For $\vs{i}{j}$ similar bound holds under the proper conditioning
\begin{equation}\label{eq:vsbound}
	\begin{split}
		\Ed\left[ \vs{i}{j} \mathbb{1}\{\widetilde{\eta} > \tau(j) \}\middle | \mathcal{G}_{\tau(j)}\right] & \le \sum_{s=j-1}^{t-1} \frac{d_s(i)}{2s}\mathbb{1}\{\widetilde{\eta} > s+1, \tau(j) = s+1\} \\
		& \le \mathbb{1}\{\widetilde{\eta} > \tau(j) \}\frac{5\log t}{C_f\phitil(i))} \wedge 1 \\
		& = q^{i,j}\mathbb{1}\{\widetilde{\eta} > \tau(j) \},
	\end{split}
\end{equation}
since $\phi(s) \le s$, for all $s$.

% Moreover, using that the random variables $\{\mathcal{U}_s\}_{s\ge 0}$ are independent from the process $\{G_t(f)\}_{t\ge 0}$, it follows that
% $$
% \Ed\left[ \es{s+1}{i}{j}\middle | \widetilde{\mathcal{F}}_s\right] = \Ed\left[ \es{s+1}{i}{j}\middle | \mathcal{F}_s\right].
% $$
% Thus, by the definition of $\est{s+1}{i}{j}$, we have that
% \begin{equation}
% 	\begin{split}
% 		\Ed\left[ \est{s+1}{i}{j}\mathbb{1}\{\widetilde{\eta} > s \}\middle | \widetilde{\mathcal{F}}_s\right] & = \mathbb{1}\{\widetilde{\eta} > s \}\left(\Ed\left[ \es{s+1}{i}{j}\middle | \mathcal{F}_s\right] +\frac{(1-\Ed\left[ \es{s+1}{i}{j}\middle | \mathcal{F}_s\right])(p_{s}^{i,j} - \Ed\left[ \es{s+1}{i}{j}\middle | \mathcal{F}_s\right])}{1-\Ed\left[ \es{s+1}{i}{j}\middle | \mathcal{F}_s\right]}\right) \\
% 		& = \mathbb{1}\{\widetilde{\eta} > s \}p_s^{i,j}.
% 	\end{split}
% \end{equation}
% Since $\mathcal{U}^{i,j}$ is also independent of $\{G_t(f)\}_{t\ge 0}$, we can argue in the same as above to obtain the identity below
% \begin{equation}
% 	\begin{split}
% 		\Ed\left[ \vst{i}{j}\mathbb{1}\{\widetilde{\eta} > \tau(j) \}\middle |  \mathcal{G}_{\tau(j)}\right] & = \mathbb{1}\{\widetilde{\eta} > \tau(j) \}q^{i,j}
% 	\end{split}
% \end{equation}

Now we will prove the upper bounds given by the statement of the lemma. We will prove the more involved cases. But first we will derive some measurability results that will play important roles in the proof latter. 

Fix $i<j<k$ and times $r<s<s'$. Observe that since $j<k$, we have $\tau(j)<\tau(k)$ and then~$\mathcal{G}_{\tau(j)} \subset \mathcal{G}_{\tau(k)}$. This implies that
\begin{equation}
	\vs{i}{j} \in \mathcal{G}_{\tau(k)}.
\end{equation}
Indeed, it is enough to notice that for a fixed $r$ and $s\ge r+1$, it follows that
\begin{align*}
	\{\tau(k) = s\}\cap \Lbrace \vs{i}{j}\mathbb{1}\{\tau(j) = r\} = 1\Rbrace = \underbrace{\{\tau(k) = s\}}_{\in \mathcal{G}_s}\cap \underbrace{\{\tau(j) = r\}}_{\in \mathcal{G}_r}\cap \underbrace{\{j\to i \text{ at time }r\}}_{\in \mathcal{G}_{r+1}\subseteq \mathcal{G}_s}, 
\end{align*}
and arguing same way to $\Lbrace \vs{i}{j}\mathbb{1}\{\tau(j) = r\} = 0\Rbrace$ implies that for any $r$, $\vs{i}{j}\mathbb{1}\{\tau(j) = r\}$ is~$\mathcal{G}_{\tau(k)}$-measurable. Consequently, $\vs{i}{j}$ is $\mathcal{G}_{\tau(k)}$-measurable as well. Also applying the same reasoning as above we also conclude that
\begin{equation}
	\vs{i}{j}\mathbb{1}\{\tau(j) = r\} \in \mathcal{F}_r.
\end{equation}
Moreover, for $r\ge s+1$ we also have that
\begin{equation}
	\es{s}{i}{j}\mathbb{1}\{\tau(k) = r\} \in \mathcal{G}_{\tau(k)}.
\end{equation}
With all the above in mind, we can prove our bounds.

\noindent \underline{Proof of item $(a)$. }
\begin{equation}\label{eq:twov}
	\begin{split}
		\Ed\left[\vs{i}{j}\vs{i}{k}\mathbb{1}\{\widetilde{\eta}>t\}\right] & = \Ed\left[ \vs{i}{j} \Ed\left[\vs{i}{k} \mathbb{1}\{\tau(k) \le t ,\widetilde{\eta}>t\}\middle | \mathcal{G}_{\tau(k)}\right] \right]\\ 
		& \le q^{i,k}\Ed\left[\vs{i}{j}\mathbb{1}\{\widetilde{\eta}>\tau(k)\}\right] \\ 
		&\le q^{i,k}\Ed\left[\vs{i}{j}\mathbb{1}\{\widetilde{\eta}>\tau(j)\}\right]\le q^{i,j}q^{i,k}.
	\end{split}
\end{equation}
The same kind of reasoning for $r<s+1$ yields
\begin{align}
	\nonumber
	\Ed\left[\vs{i}{j}\mathbb{1}\{\tau(j) = r\}\es{s+1}{j}{k}\mathbb{1}\{\widetilde{\eta}>t\}\right] & \le \Ed\left[\vs{i}{j}\mathbb{1}\{\tau(j) = r\}\Ed\left[\es{s+1}{j}{k}\mathbb{1}\{\widetilde{\eta}>s\}\middle | \mathcal{F}_s \right]\right] \\
	\label{eq:cotae1}
	& \le p_s^{j,k}\Ed\left[\vs{i}{j}\mathbb{1}\{\tau(j) = r\}\mathbb{1}\{\widetilde{\eta}>s\}\right]
\end{align}
Now, for $s+1<r\le t$ we have
\begin{align}
	\nonumber
	\Ed\left[\vs{i}{j}\mathbb{1}\{\tau(j) = r\}\es{s+1}{j}{k}\mathbb{1}\{\widetilde{\eta}>t\}\right] & \le \Ed\left[\mathbb{1}\{\tau(j) = r\}\es{s+1}{j}{k}\Ed\left[\vs{i}{j}\mathbb{1}\{\widetilde{\eta}>\tau(j)\}\middle | \mathcal{G}_{\tau(j)} \right]\right] \\
	\label{eq:cotae2}
	& \le q^{i,j}\Ed\left[\mathbb{1}\{\tau(j) = r\}\es{s+1}{j}{k}\mathbb{1}\{\widetilde{\eta}>\tau(j)\}\right].
\end{align}
Using that
$$
\Ed\left[\vs{i}{j}\es{s+1}{j}{k}\mathbb{1}\{\widetilde{\eta}>t\}\right] = \sum_{r=j}^{t}\Ed\left[\vs{i}{j}\mathbb{1}\{\tau(j) = r\}\es{s+1}{j}{k}\mathbb{1}\{\widetilde{\eta}>t\}\right]
$$
and together with \eqref{eq:cotae1} and \eqref{eq:cotae2}, leads us two
\begin{equation}\label{eq:vses}
	\begin{split}
		\Ed\left[\vs{i}{j}\es{s+1}{j}{k}\mathbb{1}\{\widetilde{\eta}>t\}\right] & \le  p_s^{j,k}\Ed\left[\vs{i}{j}\mathbb{1}\{\tau(j) \le s\}\mathbb{1}\{\widetilde{\eta}>s\}\right] + q^{i,j}\Ed\left[\mathbb{1}\{\tau(j) \ge s\}\es{s+1}{j}{k}\mathbb{1}\{\widetilde{\eta}>\tau(j)\}\right] \\
		& \le p_s^{j,k}\Ed\left[\vs{i}{j}\mathbb{1}\{\widetilde{\eta}>\tau(j)\}\right] +  q^{i,j}\Ed\left[\es{s+1}{j}{k}\mathbb{1}\{\widetilde{\eta}>s\}\right] \\
		& \le 2q^{i,j}p_s^{j,k}.
	\end{split}
\end{equation}
Observe that the above arguments make use of the time $s+1$ and the fact that $j<k$. Thus, reasoning as above we also obtain
$$
\Ed\left[\vs{i}{j}\es{s+1}{i}{k}\mathbb{1}\{\widetilde{\eta}>t\}\right] \le 2q^{i,j}p_s^{i,k}; \quad \Ed\left[\vs{i}{j}\vs{j}{k}\mathbb{1}\{\widetilde{\eta}>t\}\right] \le q^{i,j}q^{j,k}.
$$
And the same general procedure of conditioning on the `last' time also leads to
\begin{equation}
	\Ed\left[\es{r+1}{i}{j}\es{s+1}{i}{k}\mathbb{1}\{\widetilde{\eta}>t\}\right] \le p_s^{i,k}p_r^{i,j}
\end{equation}
To conclude this part of the proof, recall that by hypothesis all $i,j$ and $k$ are all greater than $10[C_f(1-\gamma)]^{-1}\log t$ and the definition of $\eta_i$. Thus, by Theorem \ref{thm:upperbounddeg2}, with $\alpha = 10[C_f(1-\gamma)]^{-1}\log t$ it follows by union bound and large enough $t$ that  
\begin{equation}
	\Pd\left( \widetilde{\eta} \le t \right) \le 6C_f^{-1}t^{-10/(1-\gamma)}.
\end{equation}
Now observe that making $i=j=t$ and using Lemma \ref{lemma:phitil} we have that
$$
p_s^{i,j}= \frac{100(\log t)^2\xi(s)^2}{[C_f(1-\gamma)]^2\widetilde{\ell}(t)^2t^{\frac{2}{1-\gamma}}}.
$$
The above observation and Proposition \ref{prop:svsmall} allow us to conclude that for all $s,r \in [1,t]$ and $i,j$ and $k$ larger than $10[C_f(1-\gamma)]^{-1}\log t$ the following bound holds
$$
6C_f^{-1}t^{-10/(1-\gamma)} \le \min\{q^{i,j}q^{i,k}, p_s^{i,j}q^{i,k}, p_s^{i,j}p_r^{i,k}\}.
$$
This is enough to conclude the proof, since, for instance
$$
\Ed\left[\vs{i}{j}\es{s+1}{j}{k}\right] \le \Ed\left[\vs{i}{j}\es{s+1}{j}{k}\mathbb{1}\{\widetilde{\eta}>t\}\right] + \Pd\left( \widetilde{\eta} \le t\right) \le  2q^{i,j}p_s^{j,k} +  q^{i,j}p_s^{j,k}.
$$
This proves part $(a)$ of our lemma.

\noindent \underline{Proof of item $(b)$.} We follow exactly the same approach we have applied for item $(a)$. Using \eqref{eq:twov} and \eqref{eq:esbound}
\begin{equation}
	\begin{split}
		\Ed \left[ \vs{i}{j}\vs{i}{k}\es{s+1}{j}{k} \mathbb{1}\{\widetilde{\eta}>t\}\right] & =	\Ed \left[ \vs{i}{j}\vs{i}{k}\es{s+1}{j}{k} \mathbb{1}\{\widetilde{\eta}>t\}\mathbb{1}\{\tau(k)\le s\}\right] \\
		& \le \Ed \left[ \vs{i}{j}\vs{i}{k} \mathbb{1}\{\widetilde{\eta}>s\}\mathbb{1}\{\tau(k)\le s\}\Ed \left[ \es{s+1}{j}{k} \middle | \mathcal{F}_s\right]\right] \\
		& \le p_{s}^{j,k}\Ed \left[ \vs{i}{j}\vs{i}{k} \mathbb{1}\{\widetilde{\eta}>s\}\mathbb{1}\{\tau(k)\le s\}\right] \\
		& = p_{s}^{j,k}\Ed \left[ \vs{i}{j}\vs{i}{k} \mathbb{1}\{\widetilde{\eta}>\tau(k)\}\right] \\
		& = p_{s}^{j,k}\Ed\left[ \vs{i}{j}  \mathbb{1}\{\widetilde{\eta}>\tau(k)\}\Ed\left[\vs{i}{k} \middle | \mathcal{G}_{\tau(k)}\right] \right]\\ 
		& \le p_{s}^{j,k}q^{i,k}q^{i,j}.
	\end{split}
\end{equation}
Reasoning as we did in the proof of item $(a)$ proves this item. This concludes the proof of the result.
\end{proof}




==> paths_l_2.tex <==
% !TeX root = ./ms.tex
\section{Bounds for the number of paths of length 2}
In this section we will provide concentration inequality results for the random variable $\cal{C}(G_t(f))$ which is defined as
\begin{equation}\label{def:Ct}
    \cal{C}(G_t(f)) := \text{number of paths of length }2 \text{ in }G_t(f).
\end{equation}
Recall that a path of length $2$ in a graph $G$ is a triplet of distinct vertices $v_1,v_2$ and $v_3$ where~$v_1\leftrightarrow v_2\leftrightarrow v_3$. 

Moreover, we do not count the paths with multiplicity, that is, a path $v_1\leftrightarrow v_2\leftrightarrow v_3$ is counted only once even though there could be multiple edges connecting each pair of vertices. For this reason, given a vertex $v$ in $G_t(f)$, we let $\Gamma_t(v)$ be the number of neighbors $v$ has in $G_t(f)$. Notice that $\Gamma_t(v) \le d_t(v)$.

The lower bound for $\mathcal{C}(G_t(f))$ relies on the existence of a vertex with a large number of neighbors. Since we will not count paths of length $2$ with multiplicity, our strategy is to prove that a high degree vertex $v$ has indeed a high number of neighbors. 
\begin{lemma}\label{lemma:neigh}Let $f$ be an edge-step function decreasing to zero. Then, for any $\varepsilon \in (0,1)$ there exist positive constants $c_1,c_2$ and $c_3$ depending on $\varepsilon$ and $f$ only such that
    $$
    \Pd \left(\exists v \in G_t(f) \; : \; \Gamma_t(v) \ge c_1F(t)t^{-\varepsilon}\right) \ge 1 - c_2t^{-c_3} - e^{-c_1F(t)/4}.
    $$
\end{lemma}
\begin{proof} By Proposition \ref{prop:grauinf}, there exist constants $c_1',c_2'$ and $c_3'$ such that $G_t(f)$ has, with probability at least $1-c_2't^{-c_3}$, a vertex $v_*$ whose degree is at least $c_1t^{1-\varepsilon}$. We denote the event of the existence of $v_*$, $A_*$. Conditioned on $A_*$, any $s \in \{t+1,\dots,2t\}$ satisfies
    \begin{equation}
        \Pd\left(U_{s} \le f(s), v_s \to v_* \mid A_* \right) = f(s)\frac{d_s(v_*)}{2s} \ge f(s)\frac{c_3't^{1-\varepsilon}}{4t} = c_3''f(s)t^{-\varepsilon}.
    \end{equation}
In words, conditioned on $A_*$, with probability at least $c_3''f(s)t^{-\varepsilon}$, at time $s$ a new vertex is added to $G_s(f)$ and this new vertex connects to $v_*$. 

Thus, conditioned on $A_*$, we have the following stochastic domination
\begin{equation}\label{eq:domination}
    N := \sum_{s=t+1}^{2t}\mathbb{1}\{U_{s} \le f(s), v_s \to v_*\} \succeq \widetilde{N} := \sum_{s=t+1}^{2t} \mathrm{Ber}\left(c_3''f(s)t^{-\varepsilon}\right),
\end{equation}
 where the Bernoulli random variables are independent among themselves. Notice that choosing $c_1$ properly and recalling $F(t)$ is increasing, we have that
 $$
\sum_{s=t+1}^{2t}c_3''f(s)t^{-\varepsilon} = c_3''t^{-\varepsilon}\left(F(2t)-F(t)\right) \ge c_1F(2t)t^{-\varepsilon}.
 $$
 A combination of Chernoff bound, the above bound and \eqref{eq:domination} leads to
 \begin{equation}
     \Pd\left( \Gamma_{2t}(v_*) \le c_1F(2t)t^{-\varepsilon}/2 \mid A_*\right) \le e^{-c_1F(2t)/8}.
 \end{equation}
 Recalling that $A^c_*$ occurs with probability at most $c_2't^{-c_3'}$ completes the proof.
\end{proof}
In order to reduce the length of some proofs and avoid clutter, we will introduce a notation for a set of indexes and state a few upper bounds for functions involving $\phi, F$ and $F^{-1}$, which will be useful latter. Let $I$ be the set of indexes below
\begin{equation}\label{def:I}
    I := \Lbrace (i,j,k) \in \N^3 \; : \; i\in \left(1,\frac{3F(t)}{2}\right), j\in \left(\frac{2F(t)}{3i}\vee i, \frac{3F(t)}{2}\right)\; k \in \left(\frac{F(t)^2}{ij}, \frac{3F(t)}{2}\right)\Rbrace.
\end{equation}
We also use the notation $\vec{i} := (i,j,k)$. In all that in mind, the lemma below will play important role in our proofs.
\begin{lemma}\label{lemma:estimativesphi} Let $f$ be an edge-step function satisfying conditions \eqref{def:conditionD0} and \eqref{def:conditionRV} for $\gamma \in [0,1)$. Then, 
   \begin{enumerate}
       \item[(a)] there exist a constant $C$, depending on $\gamma$ only, such that
        $$
            \sum_{i=i_0}^{\infty} \frac{1}{\phitil(i)^2} \le \frac{Ci_0}{\phitil(i_0)^2};
        $$
        \item[(b)] there exists a slowly varying function $\ell_1$ depending on $\gamma$ only such that
        $$
        \sum_{\vec{i} \in I}\frac{1}{\phitil(i)\phitil(j)} \le F(t)\ell_1(t);
        $$
        \item[(c)] for all $\varepsilon > 0$ and $\gamma \in (0,1)$, there exists a slowly varying function $\ell_2$ depending on $\varepsilon$ and $\gamma$ only such that
        $$
        \sum_{\vec{i} \in I}\frac{1}{\phitil(i)\phitil(j)\phitil(k)} \le \ell_2(t)t^{\varepsilon - 2\gamma}.
        $$
        \item[(d)] if $\gamma = 0$ there exists a slowly varying function $\ell_3$ such that 
        $$
        \sum_{\vec{i} \in I}\frac{1}{\phitil(i)\phitil(j)\phitil(k)} \le \ell_3(t).
        $$ 
   \end{enumerate}
    
\end{lemma}
We postpone the proof of the of the above lemma to end of this section. Now we can prove one of the main results of this section: an upper bound for the expected number of paths of length $2$.  

Due to the presence of the edge-step, paths of length $2$ can be classified according the kind of rules to build them. A path of length $2$ can be built in three different ways: via two vertex-steps, one vertex-step and one edge-step or two edge-steps. This three general categories are illustrated in the picture below, where the double arrow lines represent edges created via edge-step and the single arrow lines represent edges created via vertex-step.
\begin{figure}[h]
    \includegraphics[width=0.8 \linewidth]{images/cherries.png}
    \caption{Three types of paths of length $2$.}
\end{figure}

Observe that between vertices $i$ and $j$ can added an edge using edge-step rule any time after the insertion of $i$ and $j$. For this reason we bound the expected number of paths of length $2$ by bounding separately the expected number of each type of path. 
\begin{proposition}\label{prop:expecct}Let $f$ be an edge-step function satisfying conditions \eqref{def:conditionD0} and \eqref{def:conditionRV} for $\gamma \in [0,1)$. Then, for any $\varepsilon >0$, there exists a positive constant $C$ depending on $\gamma$ and $\varepsilon$ such that 
    $$
    \Ed\left[ \mathcal{C}(G_t)\right] \le CF(t)^2t^{\varepsilon}.
    $$
\end{proposition}
\begin{proof}  The proof will follow from a combination of Lemmas \ref{lemma:negativecor} and \ref{lemma:estimativesphi}. We first bound from above the number of paths that contains at least one vertex  smaller than $10[C_f(1-\gamma)]^{-1}\log t$. That is, we will obtain an upper bound for the following number
    $$
    \mathcal{C}_1 = \# \Lbrace i_1 \leftrightarrow i_2 \leftrightarrow  i_3 \text{ in }G_t(f)\; : \; \text{some }i\text{ is smaller than }10[C_f(1-\gamma)]^{-1}\log t\Rbrace.
    $$
    Notice that for some constant $C_1'$
    $$
    \mathcal{C}_1 \le C_1'(\log t) V^2_t(f) + C_1'^2(\log t)^2V_t(f) + C_1'^3(\log t)^3.
    $$
    Using that $V_t(f)$ is sum of $t$ independent random variables, we know by Chernoff Bounds that 
    \begin{equation}\label{eq:chernoffvt}
    \Pd\left( \frac{F(t)}{2} \le V_t(f) \le \frac{3F(t)}{2}\right) \ge 1-\exp \Lbrace - F(t)/4\Rbrace.
    \end{equation}
    Thus, we have that 
    $$
    \mathcal{C}_1 \le C_3 F(t)^2 \log t
    $$ 
    with probability at least $1-\exp \Lbrace - F(t)/4\Rbrace$ for some positive constant $C_3$ depending on $\gamma$. Since $\mathcal{C}(G_t)$ is deterministically smaller than $t^3$, it follows that
    \begin{equation}
        \Ed\left[ \mathcal{C}_1\right] \le C_3F(t)^2\log t + t^3\exp \Lbrace - F(t)/4\Rbrace \le F(t)^2\ell(t),
    \end{equation}
    where $\ell(t) = C_4 \log t$, a slowly varying function.

    Now we are left to bound the expected value of the following quantity
    \begin{equation}
        \mathcal{C}_2 = \# \Lbrace i_1 \leftrightarrow i_2 \leftrightarrow  i_3 \text{ in }G_t(f)\; : \; i_1,i_2,i_3 \ge 10[C_f(1-\gamma)]^{-1}\log t\Rbrace.
    \end{equation}
    We split $C_2$ into the following terms
    \begin{align}
        \mathcal{C}^{(0)}_2 & := \# 
        \left\{
            \begin{array}{c}
            \{i,j,k\}\subset\N\; : \; C'_f\log t<i<j<k,\; ijk\le F\left(t\right)^2
            \\ \text{ and the vertices } i,j,k \text{ form a path of length 2 in } G_t(f)  
            \end{array}
	    \right\},\\ \nonumber\\
        \mathcal{C}^{(1)}_2 & := \# 
        \left\{
            \begin{array}{c}
            \{i,j,k\}\subset\N ; C_f'\log t<i<j<k; \; ijk\ge F(t)^2
            \\ \text{ and the vertices } i,j,k \text{ form a path of length 2 in } G_t(f)  
            \\   \text{ with the two edges coming from vertex-steps}
            \end{array}
        \right\}, \\ \nonumber\\
        \mathcal{C}^{(2)}_2 & := \# 
        \left\{
            \begin{array}{c}
            \{i,j,k\}\subset\N ; C_f'\log t<i<j<k; \; ijk\ge F(t)^2
            \\ \text{ and the vertices } i,j,k \text{ form a path of length 2 in } G_t(f)  
            \\   \text{ with one edge coming from a vertex-step and another one} \\
            \text{coming from an edge-step}
            \end{array}
	    \right\}, \\ \nonumber\\
        \mathcal{C}^{(3)}_2 & := \# 
        \left\{
            \begin{array}{c}
            \{i,j,k\}\subset\N ; C_f'\log t<i<j<k; \; ijk\ge F(t)^2
            \\ \text{ and the vertices } i,j,k \text{ form a path of length 2 in } G_t(f)  
            \\   \text{ with the two edges coming from edge-steps}
            \end{array}
        \right\}
    \end{align}
    Since the above defined random variables may be sensitive to the number of vertices in the graph, expect from $\mathcal{C}_2^{(0)}$, in the next lines we will bound the expected value of $\mathcal{C}_2^{(i)}\mathbb{1}\{V_t(f) \le 3F(t)/2\}$, that is, we will control the expected number of paths of length $2$ under the event in which the number of vertices did not increase too much.

    \noindent \underline{Bound for $\mathcal{C}_2^{(0)}$:} The term $\mathcal{C}_2^{(0)}$ we bound deterministically in the following way
    \begin{equation}
        \mathcal{C}_2^{(0)} \le \sum_{i=1}^{F\left(t\right)^2}\sum_{j=1}^{F\left(t\right)^2/i}\sum_{k=1}^{F\left(t\right)^2/ij}1 \le F\left(t\right)^2 \ell_1(t),
    \end{equation}
    where $\ell_1(t)$ is the slowly varying function $(\log t)^2$.

    \noindent \underline{Bound for $\Ed\left[\mathcal{C}_2^{(1)}\mathbb{1}\{V_t(f) \le 3F(t)/2\}\right]$:}
    Notice that by Lemma \ref{lemma:negativecor} and Lemma \ref{lemma:estimativesphi} parts $(a)$ and $(b)$.
    \begin{equation}\label{eq:b1c21}
        \begin{split}
            \Ed\left[\mathcal{C}^{(1)}_2\mathbb{1}\{V_t(f)\le 3F(t)/2\}\right] & \le \Ed\left[ \sum_{\vec{i} \in I}\vs{i}{j}\vs{i}{k} + \vs{i}{j}\vs{j}{k} \right] \\
            & \le C_1\log t\sum_{\vec{i} \in I}\left(\frac{1}{\phitil(i)^2} + \frac{1}{\phitil(i)\phitil(j)} \right) \\
            & \le C'_1(\log t)F(t)^2 + C_1(\log t) \ell'_1(t)F(t) \\
            & \le \ell_2(t)F(t)^2,
        \end{split}
    \end{equation}
    where $\ell_2(t)$ is a slowly vary function. 
    
    \noindent \underline{Bound for $\Ed\left[\mathcal{C}_2^{(2)}\mathbb{1}\{V_t(f) \le 3F(t)/2\}\right]$:} First notice that following bound holds
    \begin{equation}\label{eq:b1c22}
        \begin{split}
            \Ed\left[\mathcal{C}^{(2)}_2\mathbb{1}\{V_t(f)\le 3F(t)/2\}\right] & \le \Ed\left[ \sum_{\vec{i} \in I}\sum_{s=1}^t\vs{i}{j}\es{s}{j}{k} + \vs{j}{k}\es{s}{i}{j} + \vs{i}{k}\es{s}{i}{j} \right].
        \end{split}
    \end{equation}
    Again, by Lemma \ref{lemma:negativecor}, for the first term in the RHS of the above inequality, we have
\begin{equation}\label{eq:b2c22}
    \begin{split}
        \Ed\left[ \sum_{\vec{i} \in I}\sum_{s=1}^t\vs{i}{j}\es{s}{j}{k}  \right] & \le C(\log t)^3\sum_{\vec{i} \in I}\sum_{s=1}^t \frac{1}{\phitil(i)}\frac{\phi(s)^2}{\phitil(j)\phitil(k)s^2}.
    \end{split}
\end{equation}
Since $\phi(s) = \xi(s)s$, Proposition~\ref{prop:factorout} gives us
\begin{equation}\label{eq:phi2}
    \sum_{s=1}^t \frac{\phi(s)^2}{s^2} = \sum_{s=1}^t \xi(s)^2 \le t\xi(t)^2.
\end{equation}
Here we consider $\gamma \in (0,1)$. For a small $\varepsilon <1$, a combination of the above bound with Lemma \ref{lemma:estimativesphi} part $(c)$ leads to 
\begin{equation}
    \begin{split}
        \sum_{\vec{i} \in I}\sum_{s=1}^t \frac{1}{\phitil(i)}\frac{\phi(s)^2}{\phitil(j)\phitil(k)s^2} & \le \xi(t)^2\ell'_2(t)t^{1+\varepsilon -2\gamma} \le C\xi(t)^2\ell'_2(t)F(t)^2, 
    \end{split}
\end{equation}
for some positive constant $C$, since $F(t) \sim \ell_1(t)t^{1-\gamma}/(1-\gamma)$. Finally, replacing the above bound in \eqref{eq:b2c22} gives us
\begin{equation}\label{eq:b3c22}
    \begin{split}
        \Ed\left[ \sum_{\vec{i} \in I}\sum_{s=1}^t\vs{i}{j}\es{s}{j}{k}  \right] & \le \ell_3(t)F(t)^2,
    \end{split}
\end{equation}
for some slowly varying function $\ell_3$. The same type of bound can be achieved for $\gamma = 0$ by applying part $(d)$ of Lemma \ref{lemma:estimativesphi} and noticing that in this regime $F(t) \sim f(t)t$.

\noindent \underline{Bound for $\Ed\left[\mathcal{C}_2^{(3)}\mathbb{1}\{V_t(f) \le 3F(t)/2\}\right]$:} In this case we have
\begin{equation}\label{eq:b1c23}
    \begin{split}
        \Ed\left[\mathcal{C}^{(3)}_2\mathbb{1}\{V_t(f)\le 3F(t)/2\}\right] & \le \Ed\left[ \sum_{\vec{i} \in I}\sum_{s_1=1}^t\sum_{s_2=1}^t\es{s_1}{i}{j}\es{s_2}{i}{k} + \es{s_1}{i}{j}\es{s_2}{j}{k} + \es{s_1}{i}{k}\es{s_2}{j}{k} \right].
    \end{split}
\end{equation}
By Lemma \ref{lemma:negativecor} and Equation \eqref{eq:phi2} we have the following bound
\begin{equation}
    \begin{split}
        \Ed\left[ \sum_{\vec{i} \in I}\sum_{s_1=1}^t\sum_{s_2=1}^t\es{s_1}{i}{j}\es{s_2}{i}{k} \right] &\le C(\log t)^2t^2\xi(t)^4\sum_{\vec{i} \in I}\frac{1}{\phitil(i)^2\phitil(j)\phitil(k)} \\
        & \le  \ell_4(t)t^{2+\varepsilon/2 -2\gamma}  \le CF(t)^2t^{\varepsilon}.
    \end{split}
\end{equation}
For some slowly varying function $\ell_4$ and positive constant $C$ depending on $\gamma$ and $\varepsilon$ only. In the second inequality we have used the fact that $\phitil(i)$ is increasing and goes to infinity as $i$ goes to infinity combined with items $(c)$ and $(d)$ of Lemma \ref{lemma:estimativesphi}. Whereas, for the last inequality, we have used Lemma \ref{lemma:F} and Proposition \ref{prop:svsmall}.

The other contributions on the RHS of \eqref{eq:b1c23} are bounded in the exact same way. Then, we have proven that for any $\varepsilon$ there exists $C$ such that following bound holds
$$
\Ed\left[\mathcal{C}(G_t(f))\mathbb{1}\{V_t(f)\le 3F(t)/2\}\right] \le CF(t)^2t^{\varepsilon}.
$$
Finally, by \eqref{eq:chernoffvt} and by the fact that $\mathcal{C}(G_t(f))\le t^3$ we have 
$$
\Ed\left[\mathcal{C}(G_t(f))\right] \le CF(t)^2t^{\varepsilon} + t^3\exp\{-F(t)/4\} \le C'F(t)^2t^{\varepsilon}, 
$$
which concludes the proof.
\end{proof}
The next is result provides a concentration inequality result for $\mathcal{C}(G_t(f))$ which will be useful to derive bounds for the clustering coefficient of $G_t(f)$.
\begin{theorem}[Concentration inequality for $\mathcal{C}(G_t(f))$] Let $f$ be an edge-step function satisfying conditions \eqref{def:conditionD0} and \eqref{def:conditionRV} for $\gamma \in [0,1)$. Then, for any $\varepsilon \in (0,1)$ there exist positive constants $c_1,c_2\dots, c_5$ depending on $\varepsilon$ and $f$ only such that
    $$
    \Pd \left( c_1F(t)^2t^{-\varepsilon} \le \mathcal{C}(G_t(f)) \le c_2F(t)^2t^{\varepsilon}  \right) \ge 1 - c_3t^{-c_4} - e^{-c_5F(t)}.
    $$
\end{theorem}
\begin{proof} We start by the lower bound. \\
\noindent \underline{Lower bound:}
    Observe that for any given vertex $v$ in $G_t(f)$ the following bounds hold deterministically
    \begin{equation}\label{eq:lowerbounddet}
        \mathcal{C}(G_t(f)) \ge \binom{\Gamma_t(v)}{2}.
    \end{equation}
    By Lemma \ref{lemma:neigh}, there exist a vertex $v_*$ such that 
    $$
    \Gamma_t(v_*) \ge c'_1F(t)t^{-\varepsilon}
    $$
    with probability at least $1-c'_2t^{-c'_3} - e^{-c'_1F(t)/4}$. Then, choosing $c_1$ properly and using \eqref{eq:lowerbounddet}, we conclude that
    $$
        \mathcal{C}(G_t(f)) \ge c_1F(t)^2t^{-2\varepsilon}
    $$
    with probability at least $1-c'_2t^{-c'_3} - e^{-c'_1F(t)/4}$. 

    \noindent \underline{Upper bound:} The upper bound follows by an application of Markov Inequality and Proposition \ref{prop:expecct} with $\varepsilon/2$
    $$
     \Pd\left( \mathcal{C}(G_t(f)) \ge Ct^{\varepsilon}F(t)^2 \right) \le \frac{Ct^{\varepsilon/2}F(t)^2}{Ct^{\varepsilon}F(t)^2} \le t^{-\varepsilon/2},
    $$
   which concludes the proof.
\end{proof}
We end this section proving the estimates given in Lemma \ref{lemma:estimativesphi}. It might be useful to recall the definition of the index set $I$ at Equation \eqref{def:I}.
\begin{proof}[Proof of Lemma \ref{lemma:estimativesphi}] We begin by the first item.

\noindent \underline{Part (a):} Recall that by Lemmas \ref{lemma:phixi}, \ref{lemma:finverse} and \ref{lemma:phitil}, we have the following characterization for the functions $\phi$, $F^{-1}$ and $\phitil$ 
    \begin{equation}\label{eq:phif}
        \phi(s) = \xi(s)s, \quad F^{-1}(s) = \ell(s)s^{\frac{1}{1-\gamma}}\;\text{  and  }\; \phi\left(F^{-1}(s)\right) = \phitil(s) = \widetilde{\ell}(s)s^{\frac{1}{1-\gamma}},
    \end{equation}
    where $\xi,\ell$ and $\widetilde{\ell}$ are slowly varying functions. Observe that $1/\widetilde{\ell}$ is slowly varying. Thus, by Proposition \ref{prop:sumfinite} there exists a positive constant $C$ depending on $\gamma$ only such that
    \begin{equation}\label{eq:rhs1c21}
        \begin{split}
            \sum_{i=i_0 }^\infty\frac{1}{\phitil(i)^2} & = \sum_{i = i_0 }^\infty\frac{1}{\widetilde{\ell}(i)^2i^{\frac{2}{1-\gamma}}} \le \frac{C}{\widetilde{\ell}(i_0)^2i^{\frac{1+\gamma}{1-\gamma}}_0} = \frac{Ci_0}{\phitil(i_0)^2}. 
        \end{split}
    \end{equation}

    \noindent \underline{Part (b):}  For the second part, we again make use of the identities in \eqref{eq:phif} and apply Proposition \ref{prop:sumsv} when $\gamma =0$ and Proposition \ref{prop:sumfinite} for $\gamma \in (0,1)$ to obtain
    \begin{equation}\label{eq:rhs2c21}
        \begin{split}
            \sum_{\vec{i} \in I}\frac{1}{\phitil(i)\phitil(j)} & = \sum_{\vec{i} \in I}\frac{1}{\widetilde{\ell}(i)i^{\frac{1}{1-\gamma}}\widetilde{\ell}(j)j^{\frac{1}{1-\gamma}}} \le F(t)\ell_1(t).
        \end{split}
    \end{equation}
    For $\gamma =0$ the slowly varying $\ell_1(t)$ can be taken as 
    $\left(\sum_{i=1}^t(\widetilde{\ell}(i)i)^{-1} \right)^2$ and equal to some constant~$C$ when $\gamma \in (0,1)$.
    
    \noindent \underline{Part (c):}  In this case $\gamma \in (0,1)$. In this regime Proposition \ref{prop:sumfinite} gives us a positive constant $C$ such that
    \begin{equation}\label{eq:phik}
        \begin{split}
            \sum_{ k = F(t)^2/ij}^{3F(t)/2} \frac{1}{\phitil(k)} & = \sum_{ k = F(t)^2/ij}^{3F(t)/2} \frac{1}{\widetilde{\ell}(j)j^{\frac{1}{1-\gamma}}} \le  \frac{C(ij)^{\gamma/(1-\gamma)}}{\widetilde{\ell}(F(t)^2/ij)F(t)^{2\gamma/(1-\gamma)}}
        \end{split}.
    \end{equation}
    Now, recalling that the function $1/\widetilde{\ell}$ is slowly varying, by Proposition \ref{prop:svsmall}, we have a positive constant $C$ such that for all $s\in [1,\infty)$ the following bound holds
    \begin{equation}
        \frac{1}{\widetilde{\ell}(s)} \le Cs^{\varepsilon [2(1-\gamma)]^{-1}}.
    \end{equation}
    Setting $\varepsilon'=\varepsilon/(1-\gamma)$, $a = (\varepsilon - 2\gamma)/(1-\gamma)$ and combining the above bound with identities \eqref{eq:phif} yields
    \begin{equation}
        \begin{split}
            \sum_{\vec{i} \in I}\frac{1}{\phitil(i)\phitil(j)\phitil(k)} & \le C\sum_{i=1}^{3F(t)/2}\sum_{j = 1}^{3F(t)/2}\frac{(ij)^{\gamma/(1-\gamma)}F(t)^{\varepsilon/(1-\gamma)}}{\phitil(i)\phitil(j)(ij)^{\varepsilon/(1-\gamma)}F(t)^{2\gamma/(1-\gamma)}} \\
            & \le CF(t)^{a}\sum_{i=1}^{3F(t)/2}\sum_{j = 1}^{3F(t)/2}\frac{1}{\widetilde{\ell}(i)i^{1+\varepsilon'}\widetilde{\ell}(j)j^{1+\varepsilon'}} \\
            & \le CF(t)^{(\varepsilon - 2\gamma)/(1-\gamma)} \\
            & \le Ct^{2\varepsilon -2\gamma},
        \end{split}
    \end{equation}
    where in the last inequality we used Lemma \ref{lemma:F} and Proposition \ref{prop:svsmall}. Since the choice for $\varepsilon$ was arbitrary, we conclude the proof of this part. 
    
    \noindent \underline{Part (d):}
    For $\gamma = 0$, by Proposition \ref{prop:sumsv} we have that
    \begin{equation*}
        \widehat{\ell}(t) := \sum_{k=1}^{3F(t)/2}\frac{1}{\widetilde{\ell}(k)k}
    \end{equation*}
    is a slowly varying function. Thus
    \begin{equation*}
        \begin{split}
            \sum_{\vec{i} \in I}\frac{1}{\phitil(i)\phitil(j)\phitil(k)} & \le \widehat{\ell}(t)^3,
        \end{split}
    \end{equation*}
    which is a slowly varying function.
\end{proof}

==> proof_technical_estimates.tex <==
\section{Proof of Technical Estimates}
\subsection{Time of appearance}

\begin{proof}[Proof of Lemma \ref{lemma:tauibound}]
If~$f\equiv p$, then the result follows by an elementary Bernstein bound. Assume then that~$f\in \mathrm{RES}(\gamma)$. We will prove that there exist a constant $C'_f$ such that 
\begin{equation}\label{eq:taulower}
	\P\left( \tau(i)     \leq  (1-\delta)F^{-1}(i)     \right) \le (C'_f)^{-1}\exp\left\{   -C'_f  (1-\gamma)\delta  i      \right\}.
\end{equation}
The upper bound for the probability of the event $\{\tau(i) \ge (1+\delta)F^{-1}(i)\}$ will follow from the exactly same argument.

By Theorem \ref{thm:repthm}, we know that~$f(t)=\ell(t)t^{-\gamma}$ with~$\ell$ being a slowly varying function. Proposition \ref{prop:factorout} implies that as~$r\to\infty$, using the monotonicity of~$f$ to approximate the integral by the sum,
\begin{equation}
\label{eq:cotaF2}
\begin{split}
F((1-\delta)r)
 &=\sum_{s=1}^{\lfloor  (1-\delta) r  \rfloor}      f(s)   \\  
  & =  \sum_{s=1}^{\lfloor (1-\delta) r   \rfloor}      \ell(s)s^{-\gamma}   \sim \frac{1}{1-\gamma}\ell((1-\delta) r)(1-\delta)^{1-\gamma}r^{1-\gamma} \\
  & \sim (1-\delta)^{1-\gamma} F(r),
\end{split}
\end{equation}
where we also used the fact that~$\ell$ is slowly varying to obtain~$\ell((1-\delta)r)\sim\ell(r)$. Letting $i_* = (1-\delta)F^{-1}(i)$
and recalling that~$V_r(f)$ is a sum of independent random variables, we may use the above equation, \eqref{eq:Finvdef2}, and an elementary Chernoff bound to obtain
\begin{equation}
\label{eq:tauiconc2}
\begin{split}
\lefteqn{\Pd\left(\tau(i)     \leq  (1-\delta)F^{-1}(i)     \right)}\quad\quad
\\
&=
\Pd\left( V_{i_*}(f)  \geq i     \right)
\\
&=
\Pd\left( V_{i_*}(f)  \geq \left(1+\left(i \left( F\left((1-\delta)F^{-1}(i)\right)\right)^{-1}-1\right)\right)\Ed\left[  V_{i_*}(f)       \right]    \right)
\\
&\leq 
\exp\left\{   -\frac{1}{3}   \left(i \left( F\left((1-\delta)F^{-1}(i)\right)\right)^{-1}-1\right)  F\left( (1-\delta)F^{-1}(i)\right)          \right\}
\\
&\leq 
\exp\left\{   -\frac{1}{3}  \left(   (1-\delta)^{-(1-\gamma)}      -1\right)(1-\delta)^{1-\gamma} \cdot i      \right\}
\\
&\leq 
\exp\left\{   -C(1-\gamma)\delta i      \right\},
\end{split}
\end{equation}
for sufficiently large~$i$. By adjusting the constant we can then show~\eqref{eq:taulower} for every~$i\geq 1$. 

To prove an upper bound of same order for $\Pd \left( \tau(i) \ge (1+\delta)F^{-1}(i)\right)$. Just notice the estimate given at \eqref{eq:cotaF2} also holds replacing $(1-\delta)$ by $(1+\delta)$. That is, $F(1+\delta)r) \sim (1+\delta)^{1-\gamma}F(r)$. Then, the exactly same reasoning we have done applies since the identity of events below holds
$$
\{\tau(i) \ge (1+\delta)F^{-1}(i)\} = \{V_{(1+\delta)F^{-1}(i)}(f) \le i\}.
$$
This concludes the proof.
\end{proof}
\subsection{Upper bound for the degrees}

\subsection{Number of edges between vertices: Proof of Lemma \ref{lemma:correts}}

\notarever{Enunciar já em termos de $\psi$}

Let $H$ be a simple graph, such that $V(H) \subset V(G_t(f))$ and $\edges{H} \subset \binom{V(H)}{2}$. We let $e^{H}_t$ be 
\begin{equation}
    e^{H}_t := \prod_{{i,j} \in \edges{H}}e^{ij}_t.
\end{equation}
 We write $\Hmido{i}{j}$ to denote the new graph obtained from $H$ by removing the edge $\{i,j\}$. Moreover for a vertex $i$, we will let $t_i$ be
 \begin{equation}\label{def:ti}
     t_i := F^{-1}(i).
 \end{equation}
 

\begin{lemma}\label{lemma:expectH} Let $H$ be a simple graph such that all vertices were added after time $\log^2t$ and let $\im\ge\log^2 t$ be the latest vertex appearing in $H$. Then, for $1\le s\le t$,
    \begin{equation*}\label{eq:deg2}
         \begin{split}
             \Ed \left[ e_{s}^{H}\right] & \le \sum_{\substack{i \in H, \\ \{i,\im\}\in \edges{H}}}\frac{C\log^2(t)\psi(\im)\Ed\left[e_{3t_{\im}/2}^{\Hmido{i}{\im}}\right]}{\psi(i)} + \sum_{\{i,j\} \in \edges{H}} \frac{\log^4(t)\xi^2(s)t\Ed\left[e_s^{\Hmido{i}{j}}\right]}{\psi(i)\psi(j)} + {\rm err}(t),
       \end{split}
    \end{equation*}
    where ${\rm err}(t)$ is a function of $t$ such that ${\rm err}(t) \le C't^{|\vertices{H}|^2+4}e^{-C\log^2 t}$ for any $H$.
\end{lemma}
\begin{proof} The proof is quite similar to the one given for Lemma \ref{lemma:expeijt}. For $s\ge u$, we have that, for $i,j \in H$, on the event that $i$ connects to $j$ at time $r+1$ the following identity holds
$$
\Delta e_{r}^{H}\mathbb{1} \{\tau_{\im} = u \} = e_{r}^{\Hmido{i}{j}}\mathbb{1} \{\tau_{\im} = u \}.
$$
Then, with the above identity in mind, we have that
    \begin{equation}\label{eq:t_k}
        \begin{split}
            \Ed \left[ \Delta e_{r}^{H}\mathbb{1} \{\tau_{\im} = u \} \middle | \mathcal{F}^+_{r} \right] & = \sum_{\{i,j\}\in \edges{H}} \frac{(1-Z_{r+1})e_{r}^{\Hmido{i}{j}}D_{r}(i)D_r(j)}{r^2}\mathbb{1} \{\tau_{\im} = u \}. 
        \end{split}
    \end{equation}
    To avoid clutter, let $Y_{r,u}$ and $X_{r,u}^{ij}$ be the following random variables
    \begin{equation}
        Y_{r,u} := \Delta e_{r}^{H}\mathbb{1} \{\tau_{\im} = u \}; \quad X_{r,u}^{ij}:= \frac{(1-Z_{r+1})e_{r}^{\Hmido{i}{j}}D_{r}(i)D_r(j)}{2r^2}\mathbb{1} \{\tau_{\im} = u \}.
    \end{equation}
    Recall the the definition of the event $B_t^i$ in \eqref{eq:bti} for $t>r$ and let $B_t^{H}$ be the following bad event
    \begin{equation}
        B_t^H := \bigcup_{i \in V(H)}B_t^i \implies \Pd (B_t^H) \le C'|V(H)|e^{-C \log^2(t)}.
    \end{equation}
     Moreover, for each pair of vertices $\{i,j\}\in \edges{H}$ and time $u$, recalling that at time $r$ we have at most $r+1$ vertices and edges, $X_{r,u}^{ij} \le r^{|\vertices{H}|^2}$ almost surely. 
    
    With all the above in mind and that $\phi(r)=r\xi(r)$, from \eqref{eq:t_k} we deduce the following upper bound
    \begin{equation}\label{eq:estep}
        \begin{split}
            \Ed \left[Y_{r,u}\middle | \mathcal{F}_r^+\right] & \le \sum_{\{i,j\}\in \edges{H}} X_r^{ij} \mathbb{1}_{(B^H_t)^c} + t^{|\vertices{H}|^2+2}\mathbb{1}_{B^H_t} \\
            & \le \frac{\log^4(t)\xi^2(r)r^2}{2r^2}\sum_{\{i,j\}\in \edges{H}}\frac{e_{r}^{\Hmido{i}{j}}}{\psi(i)\psi(j)}\mathbb{1} \{\tau_{\im} = u \} + t^{|\vertices{H}|^2+2}\mathbb{1}_{B^H_t},
        \end{split}
    \end{equation}
   for all $u \le r \le  t$. As in proof of Lemma \ref{lemma:expeijt}, we handle the case $r=u-1$ separately. Arguing as before by splitting the identity for the conditional expectation in terms of the indicator of $B_t^H$ and $(B_t^H)^c$, it follows that
   \begin{equation}\label{eq:vstep}
       \begin{split}
           \Ed \left[Y_{u-1,u}\middle | \mathcal{F}_{u-1}^+\right] & = \Ed \left[e^{H}_{u}\mathbb{1} \{\tau_{\im} = u \}\middle | \mathcal{F}_{u-1}^+\right]\\
           & = \sum_{\substack{i \in H, \\ \{i,\im\}\in \edges{H}}}e^{H\setminus \{i,i_M\}}_{u-1}\frac{D_{u-1}(i)\mathbb{1} \{\tau_{\im} = u \}}{2(u-1)} \\
           & \le \frac{\log^2(t)\xi(u-1)(u-1)}{2(u-1)}\sum_{\substack{i \in H, \\ \{i,\im\}\in \edges{H}}}\frac{e^{H\setminus \{i,i_M\}}_{u-1}\mathbb{1} \{\tau_{\im} = u \}}{\psi(i)}  + t^{|\vertices{H}|^2+2}\mathbb{1}_{B^H_t}.
       \end{split}
   \end{equation}
   Recalling the definition of $Y_{t,u}$ and taking the expectation on both sides of \eqref{eq:estep} and \eqref{eq:vstep} and summing over $r$ in $[u-1,s]$, with $s\le t$ lead us to the following inequality 
   \begin{equation*}
        \begin{split}
            \Ed \left[ e_{t}^{H}\mathbb{1} \{\tau_{\im} = u \} \right] & \le C't^{|\vertices{H}|^2+3}e^{-C\log^2t} + \log^2(t)\xi(u-1)\sum_{i \in H}\frac{\Ed\left[e^{H\setminus \{i,i_M\}}_{u}\mathbb{1} \{\tau_{\im} = u \}\right]}{\psi(i)} \\
            & \quad + \log^4(t)\sum_{s=1}^t\xi^2(s)\sum_{\{i,j\}\in \edges{H}} \frac{\Ed\left[e_{s}^{\Hmido{i}{j}}\mathbb{1} \{\tau_{\im} = u \} \right]}{\psi(i)\psi(j)}.
        \end{split}
   \end{equation*}
   The next step is to sum over $u$ in the range $[\im,t]$, since $e_{t}^{H}$ equals $e_{t}^{H}\mathbb{1} \{\tau_{\im} \le t \}$. In order to do that we handle each term of the RHS separately. For the first one we obtain a term which is at most $C't^{|\vertices{H}|^2+4}e^{-C\log^2t}$. As for the second term, we first recall that $\xi$ and $\phi$ are slowly varying functions with $\xi$ decreasing, which together with Lemma \ref{lemma:tauibound} imply that there exist positive constants $C'$ and $C$ depending on $f$ only such that 
   \begin{equation}
        \begin{split}
            \sum_{r=\im}^t\xi(r-1)\Ed\left[e_r^{\Hmido{i}{\im}}\mathbb{1} \{\tau_{\im} = r \}\right] & \le C'te^{-C\log^2t} + \sum_{r=t_{\im}/2}^{3t_{\im}/2}\xi(r-1)\Ed\left[e_r^{\Hmido{i}{\im}}\mathbb{1} \{\tau_{\im} = r \}\right]\\
            & \le C'te^{-C\log^2t} + C\phi(t_{\im})\Ed\left[e_{3t_{\im}/2}^{\Hmido{i}{\im}}\right].
        \end{split}
   \end{equation}
   As for the last term at the RHS, arguing similarly as we did above, using that $e_s^{\Hmido{i}{j}}\le s$,for $s\in [1,t]$, it follows that \notarever{Rever again!}
   \begin{equation}
       \sum_{r=\im}^t\Ed\left[e_s^{\Hmido{i}{j}}\mathbb{1} \{\tau_{\im} = r \}\right] \le C'te^{-C\log^2 t}+ \Ed\left[e_s^{\Hmido{i}{j}}\right].
   \end{equation}
   \notarever{Expandir} Putting all the pieces together gives us
   \begin{equation*}
       \begin{split}
             \Ed \left[ e_{t}^{H}\right] & = \Ed \left[ e_{t}^{H}\mathbb{1} \{\tau_{\im} \le t \} \right] \\
             & \le C't^3e^{-C\log^2 t}+\sum_{\substack{i \in H, \\ \{i,\im\}\in \edges{H}}}\frac{C\log^2(t)\phi(t_{\im})\Ed\left[e_{3t_{\im}/2}^{\Hmido{i}{\im}}\right]}{\psi(i)} \\
             & \quad + \sum_{\{i,j\} \in \edges{H}} \frac{\log^4(t)\xi^2(t)t\Ed\left[e_t^{\Hmido{i}{j}}\right]}{\psi(i)\psi(j)},
       \end{split}
   \end{equation*}
   which concludes the proof.
\end{proof}

Now we have all the tools we need for the proof of Lemma \ref{lemma:correts}
\begin{proof}[Proof of Lemma \ref{lemma:correts}] We will start with item (i). For vertices $i<j<k$ such that $i> \log^2(t)$, let $H$ be the path graph such that $i\sim j$ and $i\sim k$. By Lemma \ref{lemma:expectH} with $i_M = k$, and recalling that $\psi(i) = \phi(F^{-1}(i))$, we obtain
 \begin{equation}
         \begin{split}
             \Ed \left[ e_{t}^{H}\right] & \le \frac{C\log^2(t)\phi(t_{k})\Ed\left[e_{3t_{k}/2}^{jk}\right]}{\psi(i)} + \frac{C\log^2(t)\phi(t_{k})\Ed\left[e_{3t_{k}/2}^{ik}\right]}{\psi(j)}\\
             & \quad +  \frac{\log^4(t)\xi^2(t)t\Ed\left[e_t^{ik}\right]}{\psi(i)\psi(j)}+ \frac{\log^4(t)\xi^2(t)t\Ed\left[e_t^{ij}\right]}{\psi(i)\psi(k)} + {\rm err}(t).
       \end{split}
    \end{equation}
    On the other hand, by Lemma \ref{lemma:expeijt},
       \begin{equation}
           \Ed\left[e_t^{ij}\right]\le C_1t^2e^{-C_2\log^2(t)} + \frac{C_3\log^2(t)\psi(j)}{\psi(i)} + \frac{\log^4(t)t\xi^2(t)}{\phitil(i)\phitil(j)},
       \end{equation}
     \notarever{TO-DO: \\ (1) Ajustar 6.25 de $3t/2$ para $t$ usando SV e RV \\
     (2) Substituir 6.25 na ineq de cima. }
     which, for $t=t_k \ge \log(t)$, gives us that 
     \begin{equation}
         \Ed\left[e_{3t_{k}/2}^{jk}\right] \le C_1t^2e^{-C_2\log^2(t)} + \frac{C_3\log^2(t)\psi(j)}{\psi(i)} + \frac{\log^4(t)t\xi^2(t)}{\phitil(i)\phitil(j)}
     \end{equation}
\end{proof}

==> techinical_estimates.tex <==
\subsection{Time of Appearance of Vertices}
\begin{lemma}
\label{lemma:tauibound}
Consider~$f$ either in~$\mathrm{RES}(\gamma)$ with~$\gamma\in[0,1)$ or identically equal to~$p\in(0,1]$. Then there exists a constant~$C_f>0$ such that for~$i\in\N$ and every~$\delta>0$,
\begin{equation}
\label{eq:tauiconc}
\P\left((1-\delta)F^{-1}(i)\le \tau_i    \leq  (1+\delta)F^{-1}(i)     \right) \ge 1- C_f^{-1}\exp\left\{   -C_f  (1-\gamma)\delta  i      \right\}.
\end{equation}
\end{lemma}

\subsection{Upper bound for the degree}
\begin{equation}\label{def:psi}
    \psi(i) = \phi\left( F^{-1}(i)\right)
\end{equation}
\begin{theorem}\label{thm:upperbounddeg2}
	Consider~$f$ either in~$\mathrm{RES}(-\gamma)$ with~$\gamma\in[0,1)$ or identically equal to~$p\in(0,1]$. Then there exists a constant~$C_f>0$ such that, for every~$\alpha>1$,
	\begin{equation*}
	\label{eq:upperbounddeg2}
	\begin{split}
	\P\left(       \exists s\in\N \text{ such that } D_s(i) \geq   \alpha\frac{\phi(s)}{\phitil(i)}                     \right) & \leq C_f^{-1}\left(\exp\left\{   -C_f \frac{\alpha-1}{\alpha} i    \right\}     +  \exp\left\{   -C_f \cdot  \alpha    \right\} \right)    . 
	\end{split}
	\end{equation*}
\end{theorem}


\subsection{Number of edges between vertices}
\begin{lemma}\label{lemma:correts}$k>j>i>\log^2(t)$,
\begin{enumerate}
    \item[(i)] $$
        \Ed \left[ e_t^{ij}e_t^{ik} \right] \le 
    $$
    \item[(ii)]    $$
        \Ed \left[ e_t^{ij}e_t^{ik}e_t^{jk} \right] \le 
    $$ 
\end{enumerate}

 
\end{lemma}

